Learned Vertex Descent: A New Direction for 3D Human Model Fitting

We propose a novel optimization-based paradigm for 3D human model fitting on images and scans. In contrast to existing approaches that directly regress the parameters of a low-dimensional statistical body model (e.g. SMPL) from input images, we train an ensemble of per-vertex neural fields network. The network predicts, in a distributed manner, the vertex descent direction towards the ground truth, based on neural features extracted at the current vertex projection. At inference, we employ this network, dubbed LVD, within a gradient-descent optimization pipeline until its convergence, which typically occurs in a fraction of a second even when initializing all vertices into a single point. An exhaustive evaluation demonstrates that our approach is able to capture the underlying body of clothed people with very different body shapes, achieving a significant improvement compared to state-of-the-art. LVD is also applicable to 3D model fitting of humans and hands, for which we show a significant improvement to the SOTA with a much simpler and faster method.

==> section_implementation_details.tex <==

\section{Implementation details}\label{sec:implem}

\enric{Mention bilinear/trilinear interpolation}

We next describe the main implementation details. Further information is provided in the Suppl. Material and in the code that will be made publicly available.

The clipping factor for the learnt gradient is $18\%$ that of the vertical size of the scan, which we normalize between $-0.75$ and $0.75$.
In our experiments, $H=W=256$, $f$ is a stacked hourglass network~\cite{newell2016stacked} trained from scratch with 4 stacks and batch normalization replaced with group normalization~\cite{wu2018group}. 
The feature embeddings have size $128\times128$ with 256 channels each. Therefore query points have a feature size of $F = 256x4 + 3 = 1027$  \enric{I'm waiting to see if F is image features only or image features + point.}
The MLP $f$ is formed by 3 fully connected layers with Weight Normalization\cite{salimans2016weight}, and deeper architectures or positional encoding did not help to improve performance. We attribute this to the fact that the MLP is already obtaining very rich representations from feature maps. 
The networks are trained end-to-end with batch size $4$, learning rate 0.001 during 500 epochs, and then with linear learning rate decay during 500 epochs more. We use Adam Optimizer~\cite{adam} with $\beta_1=0.9$ $\beta_2=0.999$. 
When taking pointclouds as input we train an IF-Net backbone\cite{ifnet} from scratch with the same training conditions and number of iterations.

Implementation-wise $f$ has an output dimension of $N=6890$. When estimating an SMPL shape, we input a surface of $6890\times3$ and obtain a prediction of $6890\times6890\times3$, from which we sample the diagonal matrix to move each vertex in the correct direction.
